On Symmetry and the Reality of Holomorphic Hartree--Fock Wavefunctions

The coalescence and disappearance of Hartree--Fock (HF) solutions as the molecular structure varies have been a common source of criticism for the breakdown of the HF approximation to the potential energy surfaces. However, recent developments in holomorphic HF theory show that this disappearing behavior is only a manifestation of the way conventional HF equations prevent solutions from being analytically continued, but it is unclear what factors govern the existence and the locations of these disappearances. In this work, we explore some of these factors from the perspective of spatial symmetry by introducing a classification for symmetry constraints on electronic-structure calculations. This forms a framework for us to systematically investigate several analytic holomorphic HF solutions of a model $\textrm{[H}_4\textrm{]}^{2+}$ system in STO-3G and demonstrate that, under appropriate conditions, spatial symmetry imposes strict requirements on the reality of certain solutions. The implications for self-consistent-field HF search algorithms are then discussed. Throughout this article, the term reality means the quality of a holomorphic HF solution having real molecular orbitals.

==> Makefile <==
LATEXMK=latexmk
MAIN=spatialsymreality
SUPPINFO=spatialsymreality-suppinfo
TEXSOURCES:=$(MAIN).tex $(wildcard */*.tex)
TIKZSOURCES:=$(shell find -name "*.tikz")
PLOTSOURCES:=$(shell find -name "*.csv")
IMAGESOURCES:=$(shell find -name "*.eps")
SOURCES=$(TEXSOURCES) $(TIKZSOURCES) $(PLOTSOURCES) $(IMAGESOURCES) Makefile


all: $(SOURCES) notikzex-arxiv suppinfo

cleanaux:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.blg *.aux *.auxlock *.end *.fls *.log *.out *.fdb_latexmk *.synctex.gz

cleanaux-suppinfo:
	$(LATEXMK) -C $(SUPPINFO)
	rm -f $(SUPPINFO).pdfsync
	rm -rf *~ *.tmp
	rm -f *.blg *.aux *.auxlock *.end *.fls *.log *.out *.fdb_latexmk *.synctex.gz

cleanall: cleanaux cleanaux-suppinfo

notikzex-arxiv:
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O '\def\notikzex{1}\def\usecentralfigs{1}\def\twocolumnmode{1}\input{%S}'" $(MAIN).tex

suppinfo: notikzex-arxiv
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O '\def\notikzex{1}\def\noarxivcompiler{1}\input{%S}'" $(SUPPINFO).tex

suppinfo-only:
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O '\def\notikzex{1}\input{%S}'" $(SUPPINFO).tex

.PHONY: all cleanaux cleanaux-suppinfo cleanall notikzex-arxiv suppinfo


==> h4model-constraintconnections/tikz/realityregimes/regimeplot.surf.D2.c2z.all.all.tikz.tex <==
\pgfplotstableread[col sep=comma]{data/c2z/regimeplot.D2.c2z.pp.allcoarse2.allcoarse2.surf.csv}\datapp
\pgfplotstableread[col sep=comma]{data/c2z/regimeplot.D2.c2z.mp.allcoarse2.allcoarse2.surf.csv}\datamp
\pgfplotstableread[col sep=comma]{data/c2z/regimeplot.D2.c2z.mm.allcoarse2.allcoarse2.surf.csv}\datamm

\begin{tikzpicture}[
  trim axis group left,
  trim axis group right,
  ]
  \begin{groupplot}[
    % =============
    % Group configs
    % =============
    group style={
      group size=3 by 2,
      xlabels at=edge bottom,
      xticklabels at=edge bottom,
      ylabels at=edge left,
      vertical sep=0.6cm,
      horizontal sep=0.5cm,
    },
    % =================
    % Groupplot general
    % =================
    width=0.35\textwidth,
    height=0.1825\textheight,
    scale only axis,
    cycle list name=coloronly,
    unbounded coords=jump,
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    xmin=-0.003, xmax=4.003,
    ymin=0.047, ymax=5.003,
    % -----------
    % Axis labels
    % -----------
    label style={font=\footnotesize},
    xlabel={$k_2$},
    ylabel={$a / \si{\angstrom}$},
    xlabel style={align=center, font=\scriptsize},
    ylabel style={yshift=-1ex, font=\scriptsize},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\tiny},
    x tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    every x tick scale label/.style={
      at={(xticklabel* cs:1,2em)},
      anchor=north,
      inner sep=0pt,
    },
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd,
      align=right
    },
    every y tick scale label/.style={
      at={(yticklabel* cs:1.03,0.6em)},
      anchor=south east,
      inner sep=0pt,
    },
    % ------------
    % Tick configs
    % ------------
    xtick pos=left,
    xtick align=outside,
    minor x tick num=1,
    ytick pos=left,
    yticklabel pos=left,
    ytick align=outside,
    minor y tick num=1,
    ytick distance=1.0,
    % ====================
    % Colour configuration
    % ====================
    colormap/temp,
    point meta rel=per plot,
    point meta min=-2.5,
    point meta max=2.5,
  ]
    % ==============
    % ==============
    % Regime plot 2a
    % ==============
    % ==============
    % -------
    % 2a - pp
    % -------
    \nextgroupplot[
    % ===============
    % Subplot general
    % ===============
    align=center,
    % ============
    % Title format
    % ============
    title={$\left\lvert \alpha^+ \beta^+ \right\rvert$},
    title style={yshift=-1ex, font={\footnotesize}},
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    % -----------
    % Axis labels
    % -----------
    % -----------
    % Tick labels
    % -----------
    % ------------
    % Tick configs
    % ------------
    % ===========
    % Annotations
    % ===========
    after end axis/.code={
      % ============
      % D4h symmetry
      % ============
      \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
      \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
      \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
      \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
    },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datapp};
    % -------
    % 2a - mp
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha^- \beta^+ \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datamp};
    % -------
    % 2a - mm
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha^- \beta^- \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ==========
      % Colour bar
      % ==========
      colorbar,
      colorbar style={
%        at={(1.03,0.0)},
%        anchor=west,
        width=0.06*\pgfkeysvalueof{/pgfplots/parent axis width},
        height=2*\pgfkeysvalueof{/pgfplots/parent axis height}+\pgfkeysvalueof{/pgfplots/group/vertical sep},
        ylabel={$\rho$},
        ylabel style={font=\tiny, yshift=2ex},
        ytick distance=0.5,
        minor y tick num=0,
        ytick pos=both,
        ytick align=inside,
        yticklabel style={
          /pgf/number format/.cd,
          fixed,
          fixed zerofill,
          precision=1,
          /tikz/.cd,
          text width=width("$-2.5$"),
          align=right,
          xshift=-1.5ex,
        },
      },
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datamm};
    % ==============
    % ==============
    % Regime plot 2b
    % ==============
    % ==============
    % -------
    % 2b - pp
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$a / \si{\angstrom}$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datapp};
    % -------
    % 2b - mp
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datamp};
    % -------
    % 2b - mm
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin, dashed] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin] (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 2.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 3.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datamm};
  \end{groupplot}
\end{tikzpicture}

==> h4model-constraintconnections/tikz/realityregimes/regimeplot.surf.D2h.rec.sigma.all.all.tikz.tex <==
\ % !TeX root = ../../../spatialsymreality.tex

\pgfplotstableread[col sep=comma]{data/sigma/regimeplot.D2h.sigma.dashdash.allcoarse2.allcoarse2.surf.csv}\datadashdash
\pgfplotstableread[col sep=comma]{data/sigma/regimeplot.D2h.sigma.ddashdash.allcoarse2.allcoarse2.surf.csv}\dataddashdash
\pgfplotstableread[col sep=comma]{data/sigma/regimeplot.D2h.sigma.ddashddash.allcoarse2.allcoarse2.surf.csv}\dataddashddash

\begin{tikzpicture}[
  trim axis group left,
  trim axis group right,
  ]
  \begin{groupplot}[
    % =============
    % Group configs
    % =============
    group style={
      group size=3 by 2,
      xlabels at=edge bottom,
      xticklabels at=edge bottom,
      ylabels at=edge left,
      vertical sep=0.6cm,
      horizontal sep=0.5cm,
    },
    % =================
    % Groupplot general
    % =================
    width=0.35\textwidth,
    height=0.1825\textheight,
    scale only axis,
    cycle list name=coloronly,
    unbounded coords=jump,
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    xmin=0.017, xmax=2.003,
    ymin=0.047, ymax=5.003,
    % -----------
    % Axis labels
    % -----------
    label style={font=\footnotesize},
    xlabel={$k_1$},
    ylabel={$a / \si{\angstrom}$},
    xlabel style={align=center, font=\scriptsize},
    ylabel style={yshift=-1ex, font=\scriptsize},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\tiny},
    x tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    every x tick scale label/.style={
      at={(xticklabel* cs:1,2em)},
      anchor=north,
      inner sep=0pt,
    },
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd,
      align=right
    },
    every y tick scale label/.style={
      at={(yticklabel* cs:1.03,0.6em)},
      anchor=south east,
      inner sep=0pt,
    },
    % ------------
    % Tick configs
    % ------------
    xtick pos=left,
    xtick align=outside,
    minor x tick num=1,
    ytick pos=left,
    yticklabel pos=left,
    ytick align=outside,
    minor y tick num=1,
    ytick distance=1.0,
    % ====================
    % Colour configuration
    % ====================
    colormap/temp,
    point meta rel=per plot,
    point meta min=-2.5,
    point meta max=2.5,
  ]
    % ==============
    % ==============
    % Regime plot 2a
    % ==============
    % ==============
    % -------
    % 2a - dashdash
    % -------
    \nextgroupplot[
    % ===============
    % Subplot general
    % ===============
    align=center,
    % ============
    % Title format
    % ============
    title={$\left\lvert \alpha' \beta' \right\rvert$},
    title style={yshift=-1ex, font={\footnotesize}},
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    % -----------
    % Axis labels
    % -----------
    % -----------
    % Tick labels
    % -----------
    % ------------
    % Tick configs
    % ------------
    % ===========
    % Annotations
    % ===========
    after end axis/.code={
      % ============
      % D4h symmetry
      % ============
      \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
      \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
    },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datadashdash};
    % -------
    % 2a - ddashdash
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha'' \beta' \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\dataddashdash};
    % -------
    % 2a - ddashddash
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha'' \beta'' \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ==========
      % Colour bar
      % ==========
      colorbar,
      colorbar style={
%        at={(1.03,0.0)},
%        anchor=west,
        width=0.06*\pgfkeysvalueof{/pgfplots/parent axis width},
        height=2*\pgfkeysvalueof{/pgfplots/parent axis height}+\pgfkeysvalueof{/pgfplots/group/vertical sep},
        ylabel={$\rho$},
        ylabel style={font=\tiny, yshift=2ex},
        ytick distance=0.5,
        minor y tick num=0,
        ytick pos=both,
        ytick align=inside,
        yticklabel style={
          /pgf/number format/.cd,
          fixed,
          fixed zerofill,
          precision=1,
          /tikz/.cd,
          text width=width("$-2.5$"),
          align=right,
          xshift=-1.5ex,
        },
      },
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\dataddashddash};
    % ==============
    % ==============
    % Regime plot 2b
    % ==============
    % ==============
    % -------
    % 2b - dashdash
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$a / \si{\angstrom}$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datadashdash};
    % -------
    % 2b - ddashdash
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\dataddashdash};
    % -------
    % 2b - ddashddash
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\dataddashddash};
  \end{groupplot}
\end{tikzpicture}

==> h4model-constraintconnections/tikz/symbrokenregimes/regimeplot.vol.D2.tet.single.all.all.all.tikz.tex <==

\pgfplotstableread[col sep=comma]{data/c2z/regimeplot.D2.C2z.xy.single.allcoarse5.allcoarse5.allcoarse5.allxy.volume.csv}\datacz
\pgfplotstableread[col sep=comma]{data/c2z/regimeplot.D2.C2z.xy.single.single.allcoarse2.allcoarse2.allxy.volume.csv}\dataczcross

\begin{tikzpicture}[
  trim axis group left,
  trim axis group right,
  ]
  \begin{groupplot}[
    % =============
    % Group configs
    % =============
    group style={
      group size=2 by 2,
      xlabels at=edge bottom,
      xticklabels at=edge bottom,
      vertical sep=0.6cm,
      horizontal sep=1.8cm,
    },
    % =================
    % Groupplot general
    % =================
    width=0.35\textwidth,
    scale only axis,
    cycle list name=coloronly,
    unbounded coords=jump,
    view={205}{30},
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    xmin=-1, xmax=1,
    ymin=-1, ymax=1,
    zmin=+0, zmax=2,
    % -----------
    % Axis labels
    % -----------
    label style={font=\footnotesize},
    xlabel={$x$},
    zlabel={$k_2$},
    xlabel style={yshift=1.5ex, align=center, font=\scriptsize},
    ylabel style={yshift=1ex, font=\scriptsize},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\tiny},
    tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    zticklabel pos=left,
    zticklabel style={yshift=6pt},
    % ------------
    % Tick configs
    % ------------
    xtick pos=left,
    ytick pos=left,
    ztick pos=right,
    xtick align=outside,
    ytick align=outside,
    ztick align=outside,
    minor tick num=0,
    xtick distance=0.5,
    ytick distance=0.5,
    ztick distance=0.5,
    % ==========
    % Colour bar
    % ==========
    % ====================
    % Colour configuration
    % ====================
    colormap/temp,
    point meta rel=per plot,
    point meta min=-2.5,
    point meta max=+2.5,
  ]
    % ===========
    % ===========
    % Solution 2a
    % ===========
    % ===========
    % ------------------------
    % 2a - c2z - cross section
    % ------------------------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      width=0.22\textwidth,
      align=center,
      view={180}{90},
      % ============
      % Title format
      % ============
      title={$k_2 = 1$ ($\mathcal{T}_{d}$)},
      title style={font={\scriptsize}, yshift=-3pt},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      xmin=-1, xmax=1,
      ymin=-1, ymax=1,
      % -----------
      % Axis labels
      % -----------
      label style={font=\footnotesize},
      xlabel={$x$},
      ylabel={$y$},
      xlabel near ticks,
      ylabel near ticks,
      xlabel style={align=center, font=\scriptsize},
      ylabel style={yshift=-0.5ex, font=\scriptsize},
      % -----------
      % Tick labels
      % -----------
      tick label style={font=\tiny},
      xticklabel={\axisdefaultticklabel},
      x tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd
      },
      every x tick scale label/.style={
        at={(xticklabel* cs:1,2em)},
        anchor=north,
        inner sep=0pt,
      },
      y tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd,
        align=right
      },
      every y tick scale label/.style={
        at={(yticklabel* cs:1.03,0.6em)},
        anchor=south east,
        inner sep=0pt,
      },
      % ------------
      % Tick configs
      % ------------
      xtick pos=right,
      xticklabel pos=left,
      xtick align=outside,
      minor x tick num=1,
      ytick pos=right,
      yticklabel pos=right,
      ytick align=outside,
      minor y tick num=1,
      xtick distance=0.5,
      ytick distance=0.5,
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \coordinate (topcross) at (axis cs:-1,0.75,1);
      },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={x}, y={y}, meta={mlnr2a}] {\dataczcross};
    % --------
    % 2a - c2z
    % --------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      title={Pathway B, $[\hat{C}_2^{\clubsuit}]'_{xy}$ constraint},
      title style={font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ==========
      % Colour bar
      % ==========
      colorbar,
      colorbar style={
        xshift=5pt,
        width=0.06*\pgfkeysvalueof{/pgfplots/parent axis width},
        height=2*\pgfkeysvalueof{/pgfplots/parent axis height}+\pgfkeysvalueof{/pgfplots/group/vertical sep},
        ylabel={$\rho$},
        ylabel style={font=\tiny, yshift=0ex},
        ytick distance=0.5,
        minor y tick num=0,
        ytick pos=both,
        ytick align=inside,
        yticklabel style={
          /pgf/number format/.cd,
          fixed,
          fixed zerofill,
          precision=1,
          /tikz/.cd,
          text width=width("$-2.5$"),
          align=right,
          xshift=-1.5ex,
        },
      },
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \draw[->, very thin] (axis cs:1,1,-0.05) -- (axis cs:1,1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^+ \beta^+ \rvert$};
        \draw[->, very thin] (axis cs:-1,1,-0.05) -- (axis cs:-1,1,-0.4) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^- \beta^+ \rvert$};
        \draw[->, very thin] (axis cs:-1,-1,-0.05) -- (axis cs:-1,-1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^- \beta^- \rvert$};
      % =============
      % Cross-section
      % =============
      \draw[very thin] (axis cs:+1,+1,1) -- (axis cs:-1,+1,1) -- (axis cs:-1,-1,1);
      \coordinate (topcrossstart) at (axis cs:+0.75,+1,1);
      \coordinate (topcrosscontrol) at (axis cs:+0.75,+1,0.25);
      },
      ]
        \addplot3[
          scatter,
          only marks,
          mark=cube*,
          z buffer=sort,
          opacity = {0.85*\pgfplotspointmetatransformed/1000},
          point meta=explicit
        ] table[x={x}, y={y}, z={k}, meta={mlnr2a}] {\datacz};
    % ===========
    % ===========
    % Solution 2b
    % ===========
    % ===========
    % ------------------------
    % 2b - c2z - cross section
    % ------------------------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      width=0.22\textwidth,
      align=center,
      view={180}{90},
      yshift=-2cm,
      % ============
      % Title format
      % ============
      title={$k_2 = 1$ ($\mathcal{T}_{d}$)},
      title style={font={\scriptsize}, yshift=-3pt},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      xmin=-1, xmax=1,
      ymin=-1, ymax=1,
      % -----------
      % Axis labels
      % -----------
      label style={font=\footnotesize},
      xlabel={$x$},
      ylabel={$y$},
      xlabel near ticks,
      ylabel near ticks,
      xlabel style={align=center, font=\scriptsize},
      ylabel style={yshift=-0.5ex, font=\scriptsize},
      % -----------
      % Tick labels
      % -----------
      tick label style={font=\tiny},
      x tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd
      },
      every x tick scale label/.style={
        at={(xticklabel* cs:1,2em)},
        anchor=north,
        inner sep=0pt,
      },
      y tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd,
        align=right
      },
      every y tick scale label/.style={
        at={(yticklabel* cs:1.03,0.6em)},
        anchor=south east,
        inner sep=0pt,
      },
      % ------------
      % Tick configs
      % ------------
      xtick pos=right,
      xtick align=outside,
      minor x tick num=1,
      ytick pos=right,
      yticklabel pos=right,
      ytick align=outside,
      minor y tick num=1,
      xtick distance=0.5,
      ytick distance=0.5,
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \coordinate (bottomcross) at (axis cs:-1,0.75,1);
      },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={x}, y={y}, meta={mlnr2b}] {\dataczcross};
    % --------
    % 2b - c2z
    % --------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$y$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % =============
        % Cross-section
        % =============
        \draw[very thin] (axis cs:+1,+1,1) -- (axis cs:-1,+1,1) -- (axis cs:-1,-1,1);
        \coordinate (bottomcrossstart) at (axis cs:+0.75,+1,1);
        \coordinate (bottomcrosscontrol) at (axis cs:+0.75,+1,0.25);
      },
    ]
      \addplot3[
        scatter,
        only marks,
        mark=cube*,
        z buffer=sort,
        opacity = {0.85*\pgfplotspointmetatransformed/1000},
        point meta=explicit
      ] table[x={x}, y={y}, z={k}, meta={mlnr2b}] {\datacz};
  \end{groupplot}
  \draw[->, very thin] (topcrossstart) .. controls (topcrosscontrol) .. (topcross);
  \draw[->, very thin] (bottomcrossstart) .. controls (bottomcrosscontrol) .. (bottomcross);
\end{tikzpicture}

==> h4model-constraintconnections/tikz/symbrokenregimes/regimeplot.vol.D2h.rec.single.all.all.all.tikz.tex <==
\pgfplotstableread[col sep=comma]{data/i/regimeplot.D2h.i.xy.single.allcoarse5.allcoarse5.allcoarse5.allxy.volume.csv}\datai
\pgfplotstableread[col sep=comma]{data/i/regimeplot.D2h.i.xy.single.single.allcoarse2.allcoarse2.allxy.volume.csv}\dataicross
\pgfplotstableread[col sep=comma]{data/sigma/regimeplot.D2h.sigma.xy.single.allcoarse5.allcoarse5.allcoarse5.allxy.volume.csv}\datasigma

\begin{tikzpicture}[
  trim axis group left,
  trim axis group right,
  ]
  \begin{groupplot}[
    % =============
    % Group configs
    % =============
    group style={
      group size=3 by 2,
      xlabels at=edge bottom,
      xticklabels at=edge bottom,
      vertical sep=0.6cm,
      horizontal sep=1.8cm,
    },
    % =================
    % Groupplot general
    % =================
    width=0.35\textwidth,
    scale only axis,
    cycle list name=coloronly,
    unbounded coords=jump,
    view={205}{30},
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    xmin=-1, xmax=1,
    ymin=-1, ymax=1,
    zmin=+0, zmax=2,
    % -----------
    % Axis labels
    % -----------
    label style={font=\footnotesize},
    xlabel={$x$},
    zlabel={$k_1$},
    xlabel style={yshift=1.5ex, align=center, font=\scriptsize},
    ylabel style={yshift=1ex, font=\scriptsize},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\tiny},
    tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    zticklabel pos=left,
    zticklabel style={yshift=6pt},
    % ------------
    % Tick configs
    % ------------
    xtick pos=left,
    ytick pos=left,
    ztick pos=right,
    xtick align=outside,
    ytick align=outside,
    ztick align=outside,
    minor tick num=0,
    xtick distance=0.5,
    ytick distance=0.5,
    ztick distance=0.5,
    % ==========
    % Colour bar
    % ==========
    % ====================
    % Colour configuration
    % ====================
    colormap/temp,
    point meta rel=per plot,
    point meta min=-2.5,
    point meta max=+2.5,
  ]
    % ===========
    % ===========
    % Solution 2a
    % ===========
    % ===========
    % ----------------------
    % 2a - i - cross section
    % ----------------------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      width=0.22\textwidth,
      align=center,
      view={180}{90},
      % ============
      % Title format
      % ============
      title={$k_1 = 1$ ($\mathcal{D}_{4h}$)},
      title style={font={\scriptsize}, yshift=-3pt},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      xmin=-1, xmax=1,
      ymin=-1, ymax=1,
      % -----------
      % Axis labels
      % -----------
      label style={font=\footnotesize},
      xlabel={$x$},
      ylabel={$y$},
      xlabel near ticks,
      ylabel near ticks,
      xlabel style={align=center, font=\scriptsize},
      ylabel style={yshift=-0.5ex, font=\scriptsize},
      % -----------
      % Tick labels
      % -----------
      tick label style={font=\tiny},
      xticklabel={\axisdefaultticklabel},
      x tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd
      },
      every x tick scale label/.style={
        at={(xticklabel* cs:1,2em)},
        anchor=north,
        inner sep=0pt,
      },
      y tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd,
        align=right
      },
      every y tick scale label/.style={
        at={(yticklabel* cs:1.03,0.6em)},
        anchor=south east,
        inner sep=0pt,
      },
      % ------------
      % Tick configs
      % ------------
      xtick pos=right,
      xticklabel pos=left,
      xtick align=outside,
      minor x tick num=1,
      ytick pos=right,
      yticklabel pos=right,
      ytick align=outside,
      minor y tick num=1,
      xtick distance=0.5,
      ytick distance=0.5,
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \coordinate (topcross) at (axis cs:-1,0.75,1);
      },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={x}, y={y}, meta={mlnr2a}] {\dataicross};
    % ------
    % 2a - i
    % ------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      title={Pathway A, $[\hat{i}]'_{xy}$ constraint},
      title style={font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \draw[->, very thin] (axis cs:1,1,-0.05) -- (axis cs:1,1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^g \beta^g\rvert$};
        \draw[->, very thin] (axis cs:-1,1,-0.05) -- (axis cs:-1,1,-0.4) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^u \beta^g\rvert$};
        \draw[->, very thin] (axis cs:-1,-1,-0.05) -- (axis cs:-1,-1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha^u \beta^u\rvert$};
        % =============
        % Cross-section
        % =============
        \draw[very thin] (axis cs:+1,+1,1) -- (axis cs:-1,+1,1) -- (axis cs:-1,-1,1);
        \coordinate (topcrossstart) at (axis cs:+0.75,+1,1);
        \coordinate (topcrosscontrol) at (axis cs:+0.75,+1,0.25);
      },
    ]
      \addplot3[
        scatter,
        only marks,
        mark=cube*,
        z buffer=sort,
        opacity = {0.85*\pgfplotspointmetatransformed/1000},
        point meta=explicit
      ] table[x={x}, y={y}, z={k}, meta={mlnr2a}] {\datai};
    % ----------
    % 2a - sigma
    % ----------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      title={Pathway A, $\left[\hat{\sigma}^{xz}\right]'_{xy}$ constraint},
      title style={font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ==========
      % Colour bar
      % ==========
      colorbar,
      colorbar style={
        xshift=5pt,
        width=0.06*\pgfkeysvalueof{/pgfplots/parent axis width},
        height=2*\pgfkeysvalueof{/pgfplots/parent axis height}+\pgfkeysvalueof{/pgfplots/group/vertical sep},
        ylabel={$\rho$},
        ylabel style={font=\tiny, yshift=0ex},
        ytick distance=0.5,
        minor y tick num=0,
        ytick pos=both,
        ytick align=inside,
        yticklabel style={
          /pgf/number format/.cd,
          fixed,
          fixed zerofill,
          precision=1,
          /tikz/.cd,
          text width=width("$-2.5$"),
          align=right,
          xshift=-1.5ex,
        },
      },
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \draw[->, very thin] (axis cs:1,1,-0.05) -- (axis cs:1,1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha' \beta' \rvert$};
        \draw[->, very thin] (axis cs:-1,1,-0.05) -- (axis cs:-1,1,-0.4) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha'' \beta' \rvert$};
        \draw[->, very thin] (axis cs:-1,-1,-0.05) -- (axis cs:-1,-1,-0.6) node[inner sep=2pt, scale=0.5, anchor=north] {$\lvert \alpha'' \beta'' \rvert$};
      },
      ]
        \addplot3[
          scatter,
          only marks,
          mark=cube*,
          z buffer=sort,
          opacity = {0.85*\pgfplotspointmetatransformed/1000},
          point meta=explicit
        ] table[x={x}, y={y}, z={k}, meta={mlnr2a}] {\datasigma};
    % ===========
    % ===========
    % Solution 2b
    % ===========
    % ===========
    % ----------------------
    % 2b - i - cross section
    % ----------------------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      width=0.22\textwidth,
      align=center,
      view={180}{90},
      yshift=-2cm,
      % ============
      % Title format
      % ============
      title={$k_1 = 1$ ($\mathcal{D}_{4h}$)},
      title style={font={\scriptsize}, yshift=-3pt},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      xmin=-1, xmax=1,
      ymin=-1, ymax=1,
      % -----------
      % Axis labels
      % -----------
      label style={font=\footnotesize},
      xlabel={$x$},
      ylabel={$y$},
      xlabel near ticks,
      ylabel near ticks,
      xlabel style={align=center, font=\scriptsize},
      ylabel style={yshift=-0.5ex, font=\scriptsize},
      % -----------
      % Tick labels
      % -----------
      tick label style={font=\tiny},
      x tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd
      },
      every x tick scale label/.style={
        at={(xticklabel* cs:1,2em)},
        anchor=north,
        inner sep=0pt,
      },
      y tick label style={
        /pgf/number format/.cd,
        fixed,
        fixed zerofill,
        precision=1,
        /tikz/.cd,
        align=right
      },
      every y tick scale label/.style={
        at={(yticklabel* cs:1.03,0.6em)},
        anchor=south east,
        inner sep=0pt,
      },
      % ------------
      % Tick configs
      % ------------
      xtick pos=right,
      xtick align=outside,
      minor x tick num=1,
      ytick pos=right,
      yticklabel pos=right,
      ytick align=outside,
      minor y tick num=1,
      xtick distance=0.5,
      ytick distance=0.5,
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        \coordinate (bottomcross) at (axis cs:-1,0.75,1);
      },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={x}, y={y}, meta={mlnr2b}] {\dataicross};
    % ------
    % 2b - i
    % ------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$y$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % =============
        % Cross-section
        % =============
        \draw[very thin] (axis cs:+1,+1,1) -- (axis cs:-1,+1,1) -- (axis cs:-1,-1,1);
        \coordinate (bottomcrossstart) at (axis cs:+0.75,+1,1);
        \coordinate (bottomcrosscontrol) at (axis cs:+0.75,+1,0.25);
      },
    ]
      \addplot3[
        scatter,
        only marks,
        mark=cube*,
        z buffer=sort,
        opacity = {0.85*\pgfplotspointmetatransformed/1000},
        point meta=explicit
      ] table[x={x}, y={y}, z={k}, meta={mlnr2b}] {\datai};
    % ----------
    % 2b - sigma
    % ----------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      % height=.1825\textheight,
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$y$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
      },
    ]
      \addplot3[
        scatter,
        only marks,
        mark=cube*,
        z buffer=sort,
        opacity = {0.85*\pgfplotspointmetatransformed/1000},
        point meta=explicit
      ] table[x={x}, y={y}, z={k}, meta={mlnr2b}] {\datasigma};
  \end{groupplot}
  \draw[->, very thin] (topcrossstart) .. controls (topcrosscontrol) .. (topcross);
  \draw[->, very thin] (bottomcrossstart) .. controls (bottomcrosscontrol) .. (bottomcross);
\end{tikzpicture}

==> h4model-solutions/tikz/realityregimes/regimeplot.surf.D2h.rec.i.all.all.tikz.tex <==
\ % !TeX root = ../../../spatialsymreality.tex

\pgfplotstableread[col sep=comma]{data/i/regimeplot.D2h.i.gg.allcoarse2.allcoarse2.surf.csv}\datagg
\pgfplotstableread[col sep=comma]{data/i/regimeplot.D2h.i.ug.allcoarse2.allcoarse2.surf.csv}\dataug
\pgfplotstableread[col sep=comma]{data/i/regimeplot.D2h.i.uu.allcoarse2.allcoarse2.surf.csv}\datauu

\begin{tikzpicture}[
  trim axis group left,
  trim axis group right,
  ]
  \begin{groupplot}[
    % =============
    % Group configs
    % =============
    group style={
      group size=3 by 2,
      xlabels at=edge bottom,
      xticklabels at=edge bottom,
      ylabels at=edge left,
      vertical sep=0.6cm,
      horizontal sep=0.6cm,
    },
    % =================
    % Groupplot general
    % =================
    width=0.29\textwidth,
    height=0.1825\textheight,
    scale only axis,
    cycle list name=coloronly,
    unbounded coords=jump,
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    xmin=0.017, xmax=2.003,
    ymin=0.047, ymax=5.003,
    % -----------
    % Axis labels
    % -----------
    label style={font=\footnotesize},
    xlabel={$k_1$},
    ylabel={$a / \si{\angstrom}$},
    xlabel style={align=center, font=\scriptsize},
    ylabel style={yshift=-1ex, font=\scriptsize},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\tiny},
    x tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    every x tick scale label/.style={
      at={(xticklabel* cs:1,2em)},
      anchor=north,
      inner sep=0pt,
    },
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd,
      align=right
    },
    every y tick scale label/.style={
      at={(yticklabel* cs:1.03,0.6em)},
      anchor=south east,
      inner sep=0pt,
    },
    % ------------
    % Tick configs
    % ------------
    xtick pos=left,
    xtick align=outside,
    minor x tick num=1,
    ytick pos=left,
    yticklabel pos=left,
    ytick align=outside,
    minor y tick num=1,
    ytick distance=1.0,
    % ====================
    % Colour configuration
    % ====================
    colormap/temp,
    point meta rel=per plot,
    point meta min=-2.5,
    point meta max=2.5,
  ]
    % ==============
    % ==============
    % Regime plot 2a
    % ==============
    % ==============
    % -------
    % 2a - gg
    % -------
    \nextgroupplot[
    % ===============
    % Subplot general
    % ===============
    align=center,
    % ============
    % Title format
    % ============
    title={$\left\lvert \alpha^g \beta^g \right\rvert$},
    title style={yshift=-1ex, font={\footnotesize}},
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
    % -----------
    % Axis labels
    % -----------
    % -----------
    % Tick labels
    % -----------
    % ------------
    % Tick configs
    % ------------
    % ===========
    % Annotations
    % ===========
    after end axis/.code={
      % ============
      % D4h symmetry
      % ============
      \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
      \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
    },
    ]
      \addplot[
        surf,
        mesh/rows=101,
        mesh/ordering=x varies,
        patch type=bilinear,
        shader=interp,
        mesh input=lattice,
        point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datagg};
    % -------
    % 2a - ug
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha^u \beta^g \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\dataug};
    % -------
    % 2a - uu
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      title={$\left\lvert \alpha^u \beta^u \right\rvert$},
      title style={yshift=-1ex, font={\footnotesize}},
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ==========
      % Colour bar
      % ==========
      colorbar,
      colorbar style={
%        at={(1.03,0.0)},
%        anchor=west,
        width=0.06*\pgfkeysvalueof{/pgfplots/parent axis width},
        height=2*\pgfkeysvalueof{/pgfplots/parent axis height}+\pgfkeysvalueof{/pgfplots/group/vertical sep},
        ylabel={$\rho$},
        ylabel style={font=\tiny, yshift=2ex},
        ytick distance=0.5,
        minor y tick num=0,
        ytick pos=both,
        ytick align=inside,
        yticklabel style={
          /pgf/number format/.cd,
          fixed,
          fixed zerofill,
          precision=1,
          /tikz/.cd,
          text width=width("$-2.5$"),
          align=right,
          xshift=-1.5ex,
        },
      },
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
      ]
        \addplot[
          surf,
          mesh/rows=101,
          mesh/ordering=x varies,
          patch type=bilinear,
          shader=interp,
          mesh input=lattice,
          point meta=explicit
        ] table[x={k}, y={aHH}, meta={mlnr2a}] {\datauu};
    % ==============
    % ==============
    % Regime plot 2b
    % ==============
    % ==============
    % -------
    % 2b - gg
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      ylabel={$a / \si{\angstrom}$},
      % -----------
      % Tick labels
      % -----------
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datagg};
    % -------
    % 2b - ug
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\dataug};
    % -------
    % 2b - uu
    % -------
    \nextgroupplot[
      % ===============
      % Subplot general
      % ===============
      align=center,
      % ============
      % Title format
      % ============
      % ===========
      % Axis format
      % ===========
      % -----------
      % Axis scales
      % -----------
      % -----------
      % Axis labels
      % -----------
      % -----------
      % Tick labels
      % -----------
      yticklabels={,,},
      % ------------
      % Tick configs
      % ------------
      % ===========
      % Annotations
      % ===========
      after end axis/.code={
        % ============
        % D4h symmetry
        % ============
        \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
        \draw[gray, very thin, dashed] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},1.058350) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},1.058350);
      },
    ]
      \addplot[
      surf,
      mesh/rows=101,
      mesh/ordering=x varies,
      patch type=bilinear,
      shader=interp,
      mesh input=lattice,
      point meta=explicit
      ] table[x={k}, y={aHH}, meta={mlnr2b}] {\datauu};
  \end{groupplot}
\end{tikzpicture}

==> introduction/tikz/H42p.STO-3G.UHF.a1.058350.tikz.tex <==
\ % !TeX root=../../../spatialsymreality.tex

\pgfplotstableread[col sep=comma]{introduction/data/H42p.STO-3G.UHF.a1.058350.csv}\data

\newlength{\molsize}
\setlength{\molsize}{1.1cm}
\begin{tikzpicture}[%
  trim axis left,%
  trim axis right,%
]
  \begin{axis}[
    % =======
    % General
    % =======
    height=21cm,
    width=.83\textwidth,
    align=center,
    cycle list name=coloronly,
    unbounded coords=jump,
    % ============
    % Title format
    % ============
    % ===========
    % Axis format
    % ===========
    % -----------
    % Axis scales
    % -----------
%    scaled x ticks=false,
%    scaled y ticks=base 10:3,
    restrict x to domain=0.6:1.4,
    xmin=0.70, xmax=1.30,
    restrict y to domain=-1:1,
    ymin=-0.9, ymax=0.9,
    % -----------
    % Axis labels
    % -----------
    xlabel={$k_1$},
    ylabel={Energy / $\si{\hartree}$},
    label style={font=\small},
    xlabel style={align=center},
    ylabel style={yshift=0ex},
    % -----------
    % Tick labels
    % -----------
    tick label style={font=\small},
    y tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=1,
      /tikz/.cd
    },
    x tick label style={
      /pgf/number format/.cd,
      fixed,
      fixed zerofill,
      precision=2,
      /tikz/.cd
    },
    % ------------
    % Tick configs
    % ------------
%    y tick num=3,
    xtick pos=left,
    ytick pos=both,
    yticklabel pos=left,
    xtick align=outside,
    ytick align=outside,
    minor x tick num=1,
    minor y tick num=1,
%    xtick distance=15,
%    ytick distance=0.001,
    % =============
    % Legend format
    % =============
    % ===========
    % Annotations
    % ===========
    after end axis/.code={
      % ==========
      % UHF labels
      % ==========
      % -----------
      % A solutions
      % -----------
      \node[anchor=north east, inner sep=1pt, scale=1] (A) at (axis cs:0.775,-0.80) {$\mathrm{A}$};
      % -----------
      % B solutions
      % -----------
      \node[anchor=north east, inner sep=1pt, scale=1] (B) at (axis cs:0.99,-0.45) {$\mathrm{B}$};
      \pgfplotstablegetelem{23}{i.ug.3a}\of{\data}
      \draw[->, very thin] (axis cs:1,\pgfplotsretval) -- (B);
      \node[anchor=north east, inner sep=1pt, scale=1] (Bd) at (axis cs:0.775,-0.14) {$\mathrm{B}'$};
      \node[anchor=north east, inner sep=1pt, scale=1] (Bdd) at (axis cs:0.775,-0.36) {$\mathrm{B}''$};
      % -----------
      % C solutions
      % -----------
      \node[anchor=north west, inner sep=1pt, scale=1] (C) at (axis cs:1.05,-0.09) {$\mathrm{C}$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Cd) at (axis cs:0.775,0.305) {$\mathrm{C}'$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Cdd) at (axis cs:0.775,0.55) {$\mathrm{C}''$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Ctd) at (axis cs:0.775,0.12) {$\mathrm{C}'''$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Cqd) at (axis cs:0.775,0.415) {${\mathrm{C}^{4}}'$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Cqnd) at (axis cs:1.05,0.10) {${\mathrm{C}^{5}}'$};
      % -----------
      % D solutions
      % -----------
      \node[anchor=south west, inner sep=1pt, scale=1] (D) at (axis cs:0.89,0.8) {$\mathrm{D}$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Dd) at (axis cs:0.85,0.755) {$\mathrm{D}'$};
      \node[anchor=south west, inner sep=1pt, scale=1] (Ddd) at (axis cs:1.02,0.62) {$\mathrm{D}''$};
      \pgfplotstablegetelem{29}{i.ug.2a}\of{\data}
      \draw[->, very thin] (axis cs:1,\pgfplotsretval) -- (Ddd);
      % -----------
      % E solutions
      % -----------
      \node[anchor=south west, inner sep=1pt, scale=1] (E) at (axis cs:1.20,0.82) {$\mathrm{E}$};
      % ==================
      % Coalescence points
      % ==================
      % -------
      % i.ug.2a (short, top)
      % -------
      \pgfplotstablegetelem{0}{i.ug.2a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:0.9725988567,\pgfplotsretval) {};
      \pgfplotstablegetelem{61}{i.ug.2a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:1.0302357443,\pgfplotsretval) {};
      % -------
      % i.ug.3a (short, bottom)
      % -------
      \pgfplotstablegetelem{0}{i.ug.3a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:0.9782680588,\pgfplotsretval) {};
      \pgfplotstablegetelem{50}{i.ug.3a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:1.0255114093,\pgfplotsretval) {};
      % -------
      % i.uu.2a (long, top)
      % -------
      \pgfplotstablegetelem{0}{i.uu.2a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:0.8771672887,\pgfplotsretval) {};
      \pgfplotstablegetelem{72}{i.uu.2a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:1.2173194123,\pgfplotsretval) {};
      % -------
      % i.uu.3a (long, bottom)
      % -------
      \pgfplotstablegetelem{0}{i.uu.3a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:0.8214201351,\pgfplotsretval) {};
      \pgfplotstablegetelem{90}{i.uu.3a}\of{\data}
      \node[circle, fill=red, draw=black, inner sep=1.75pt] at (axis cs:1.2456654226,\pgfplotsretval) {};
      % =====================
      % Parameter definitions
      % =====================
      \coordinate (molecule) at (axis cs:1.15,-0.7);
      \node[draw, shape=circle, fill=gray, scale=0.5] (H1) at ($(molecule) + (-0.75\molsize,0.55\molsize)$) {};
      \node[draw, shape=circle, fill=gray, scale=0.5] (H2) at ($(molecule) + (0.75\molsize,0.55\molsize)$) {};
      \node[draw, shape=circle, fill=gray, scale=0.5] (H3) at ($(molecule) + (0.75\molsize,-0.55\molsize)$) {};
      \node[draw, shape=circle, fill=gray, scale=0.5] (H4) at ($(molecule) + (-0.75\molsize,-0.55\molsize)$) {};
      \draw (H1) -- (H2) -- (H3) -- (H4) -- (H1) -- cycle;
      \node[inner sep=3pt, scale=0.9, anchor=east] (a) at ($(H1)!.5!(H4)$) {$a$};
      \node[inner sep=3pt, scale=0.9, anchor=north] (ka) at ($(H3)!.5!(H4)$) {$k_1a$};
      % =========
      % Zero axis
      % =========
%      \draw[gray, very thin] (axis cs: \pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs: \pgfkeysvalueof{/pgfplots/xmax},0);
      % ====================
      % Point-group symmetry
      % ====================
      % ---
      % D4h
      % ---
      \draw[gray, very thin] (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs: 1.0,\pgfkeysvalueof{/pgfplots/ymax});
      \node[anchor=south, inner sep=3pt] (D4h) at ($(axis cs:1,\pgfkeysvalueof{/pgfplots/ymax}) + (0,3)$) {$\mathcal{D}_{4h}$};
      \node[anchor=south, inner sep=3pt] (D2hleft) at ($(axis cs:0.875,\pgfkeysvalueof{/pgfplots/ymax}) + (0,3)$) {$\mathcal{D}_{2h}$};
      \node[anchor=south, inner sep=3pt] (D2hright) at ($(axis cs:1.125,\pgfkeysvalueof{/pgfplots/ymax}) + (0,3)$) {$\mathcal{D}_{2h}$};
      \draw[-] ($(D4h.west) + (-12,0)$) -- ($(D2hleft.east) + (12,0)$);
      \draw[->] ($(D2hleft.west) + (-12,0)$) -- ({D2hleft} -| {axis cs: \pgfkeysvalueof{/pgfplots/xmin},0.9});
      \draw[-] ($(D4h.east) + (+12,0)$) -- ($(D2hright.west) + (-12,0)$);
      \draw[->] ($(D2hright.east) + (12,0)$) -- ({D2hright} -| {axis cs: \pgfkeysvalueof{/pgfplots/xmax},0.9});
    },
  ]
    \foreach \prealscf in {i.gg.1a, i.gg.1b, i.gg.1d, i.ug.1a, i.ug.1b, i.ug.1c, i.ug.1d, i.uu.1a, i.uu.1b, i.uu.1d}{
      \addplot+[thick, mark=none] table[x={k1}, y={\prealscf}]{\data};
    }
    \foreach \trealscf in {i.ug.2a, i.ug.3a, i.uu.2a, i.uu.3a}{
      \addplot+[densely dashed, very thick, mark=none] table[x={k.\trealscf}, y={\trealscf}]{\data};
    }
  \end{axis}
\end{tikzpicture}

==> spatialsymrealityaux.tex <==



==> suppinfo/Makefile <==
LATEXMK=latexmk
MAIN=spatialsymreality-suppinfo
TEXSOURCES:=$(MAIN).tex $(wildcard */*.tex)
TIKZSOURCES:=$(shell find -name "*.tikz")
PLOTSOURCES:=$(shell find -name "*.csv")
IMAGESOURCES:=$(shell find -name "*.eps")
SOURCES=$(TEXSOURCES) $(TIKZSOURCES) $(PLOTSOURCES) $(IMAGESOURCES) Makefile


all: $(SOURCES) notikzex

cleanaux:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.bib *.blg *.aux *.auxlock *.end *.fls *.log *.out *.fdb_latexmk *.synctex.gz

cleanall: cleanaux

tikzex:
	$(LATEXMK) -quiet -lualatex \
			-pdflualatex="lualatex --shell-escape --synctex=1 --interaction=nonstopmode %O %S" $(MAIN).tex

notikzex:
	$(LATEXMK) -quiet -pdf \
			-pdflatex="pdflatex --shell-escape --synctex=1 --interaction=nonstopmode %O '\def\notikzex{1}\input{%S}'" $(MAIN).tex

.PHONY: all cleanaux cleanall tikzex notikzex

